Parameterized Concurrent Multi-Party Session Types

Session types have been proposed as a means of statically verifying implementations of communication protocols. Although prior work has been successful in verifying some classes of protocols, it does not cope well with parameterized, multi-actor scenarios with inherent asynchrony. For example, the sliding window protocol is inexpressible in previously proposed session type systems. This paper describes System-A, a new typing language which overcomes many of the expressiveness limitations of prior work. System-A explicitly supports asynchrony and parallelism, as well as multiple forms of parameterization. We define System-A and show how it can be used for the static verification of a large class of asynchronous communication protocols.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{Natallia Kokash and Ant\'onio Ravara (Eds.): 11th International Workshop on\\ Foundations of Coordination Languages and Self Adaptation (FOCLASA'12)\\
EPTCS 91, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.91.2}{10.4204/EPTCS.91.2}}
\pdfoutput=1

